Representing Affect Information in Word Embeddings

A growing body of research in natural language processing (NLP) and natural language understanding (NLU) is investigating human-like knowledge learned or encoded in the word embeddings from large language models. This is a step towards understanding what knowledge language models capture that resembles human understanding of language and communication. Here, we investigated whether and how the affect meaning of a word (i.e., valence, arousal, dominance) is encoded in word embeddings pre-trained in large neural networks. We used the human-labeled dataset as the ground truth and performed various correlational and classification tests on four types of word embeddings. The embeddings varied in being static or contextualized, and how much affect specific information was prioritized during the pre-training and fine-tuning phase. Our analyses show that word embedding from the vanilla BERT model did not saliently encode the affect information of English words. Only when the BERT model was fine-tuned on emotion-related tasks or contained extra contextualized information from emotion-rich contexts could the corresponding embedding encode more relevant affect information.

==> Affect embeddings/Preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% AUTHORS: DO NOT EDIT PLEASE %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% ------------ Preamble.tex for ELM-proceedings-template.tex  -- ELM proceedings template ---------------------------------------------------------------------------
% Adapted by Alex Kalomoiros and Florian Schwarz from the  LSA Proceedings template created by Sarah E. Murray.
% http://journals.linguisticsociety.org/proceedings/index.php/PLSA/pages/view/instructions

\usepackage{leipzig}
\usepackage{tipa} %The tipa package, if used, needs to be placed before linguex, to avoid formatting issues.
\usepackage{graphicx}
\usepackage{linguex}
\usepackage{multirow}

% documentation at http://texdoc.net/texmf-dist/doc/latex/linguex/linguex-doc.pdf


\usepackage{enumitem}
\setlist{noitemsep, topsep=6pt} % removes spacing between list items; sets 6pt space above list

%---------------------------------------------------------------------------
\usepackage{times}
\usepackage{natbib}	
\setcitestyle{comma,aysep={},yysep={,},notesep={; }}
 \setlength{\bibsep}{0.0pt}
\usepackage{fullpage} 
\usepackage[compact]{titlesec}
	\titleformat{\section}[runin]{\normalfont\bfseries}{\thesection.}{.5em}{}[.]
	\titleformat{\subsection}[runin]{\normalfont\scshape}{\thesubsection.}{.5em}{}[.]
	\titleformat{\subsubsection}[runin]{\normalfont\scshape}{\thesubsubsection.}{.5em}{}[.]
\usepackage[usenames,dvipsnames]{color}	
\definecolor{splinkcolor}{rgb}{.0,.2,.4}
\usepackage[colorlinks,allcolors={black},urlcolor={splinkcolor}]{hyperref} 		%likes to be last package %this isn't the exact color as in the LSA stylesheet, but this (need color package) or cyan (predefined) seems close enough



% -------------- LSA definitions ---------------------------------------------------------------------------------------------------------           
\setlength\parindent{0.3in}			%paragraphs indented 0.3inches
\setlength\intextsep{6pt}			%spacing before and after tables
\setlength\abovecaptionskip{6pt}	%spacing between figure and caption

\usepackage[vskip=6pt,leftmargin=0.3in,rightmargin=0.3in,indentfirst=false]{quoting}


%-------------------------------------------------------------- format title --------------------------------------
\makeatletter
\def\@maketitle{%
  \newpage
  \begin{center}%
  \let \footnote \thanks
    {\normalfont\bfseries \@title \par}%
    {\vskip .5em%\vskip 6pt%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
  \end{center}%
  \par}
\makeatother
%-------------------------------------------------------------- format abstract environment --------------------------------------
% Abstracts have to be 12pt, indented 1.4 inches on each side, and inline with the label
\renewenvironment{abstract}{%
\noindent\begin{minipage}{1\textwidth}
\setlength{\leftskip}{0.4in}
\setlength{\rightskip}{0.4in}
\textbf{Abstract.}}
{\end{minipage}}
%-------------------------------------------------------------- format keywords environment --------------------------------------
% Abstracts have to be 12pt, indented 1.4 inches on each side, and inline with the 
\newenvironment{keywords}{%
\vspace{.5em}
\noindent\begin{minipage}{1\textwidth}
\setlength{\leftskip}{0.4in}
\setlength{\rightskip}{0.4in}
\textbf{Keywords.}}
{\end{minipage}}




\pagestyle{empty}
